A Survey on Human-Centric LLMs

The rapid evolution of large language models (LLMs) and their capacity to simulate human cognition and behavior has given rise to LLM-based frameworks and tools that are evaluated and applied based on their ability to perform tasks traditionally performed by humans, namely those involving cognition, decision-making, and social interaction. This survey provides a comprehensive examination of such human-centric LLM capabilities, focusing on their performance in both individual tasks (where an LLM acts as a stand-in for a single human) and collective tasks (where multiple LLMs coordinate to mimic group dynamics). We first evaluate LLM competencies across key areas including reasoning, perception, and social cognition, comparing their abilities to human-like skills. Then, we explore real-world applications of LLMs in human-centric domains such as behavioral science, political science, and sociology, assessing their effectiveness in replicating human behaviors and interactions. Finally, we identify challenges and future research directions, such as improving LLM adaptability, emotional intelligence, and cultural sensitivity, while addressing inherent biases and enhancing frameworks for human-AI collaboration. This survey aims to provide a foundational understanding of LLMs from a human-centric perspective, offering insights into their current capabilities and potential for future development.

==> LLM_table_draft.tex <==


\begin{table}[ht]
\centering
\newcolumntype{L}[1]{>{\raggedright\arraybackslash}p{#1}}
\newcolumntype{Y}{>{\raggedright\arraybackslash}X} % New column type for text wrapping
\scriptsize 
\vspace*{-5px}

\caption{Review of LLM Competency Evaluation Papers}
\vspace*{-5px}

\resizebox{\textwidth}{!}{%
\begin{tabular}{p{2cm}p{2cm}p{0.6cm}p{0.6cm}p{3.8cm}p{6.4cm}p{3.2cm}p{1.2cm}}
% {@{}cccccccc@{}}

\toprule
\textbf{Category}  & \textbf{Skill}  & \textbf{Paper} & \textbf{Year} & \textbf{LLM(s) Used} & \textbf{Contribution} & \textbf{Evaluation Metrics}& \textbf{Compared to Human}
  \\ \midrule
\multirow{2}{*}{Cognitive Skills} 
                           & Reasoning &   \cite{liu2023logiqa}             & 2023         & GPT-2, GPT-3                           &       Introduces LogiQA 2.0 dataset for evaluating LLM’s capabilities in complex logical reasoning       &   Accuracy, precision, recall, and F1-score   &   \ding{51}                                                        \\ \cmidrule(l){3-8} 
                          &   &   \cite{saparov2022language}                      & 2022       & InstructGPT, GPT-3         &  Creates PrOntoQA, a first-order logic-based synthetic dataset designed to analyze LLMs’ reasoning abilities by converting their chain-of-thought prompts into symbolic proofs         &    Strict to more relaxed version of proof accuracy    & \ding{55}            \\ \cmidrule(l){3-8}

                           &   &   \cite{talmor2022commonsenseqa}                      & 2022       &  T5, UNICORN, GPT-3     &  Designs CommonsenseQA 2.0, a gamification-based benchmark, for exploring AI common sense limits & Accuracy, consistency                  & \ding{51}            \\  \cmidrule(l){3-8} 
                           
                          &   &   \cite{onoe2021creak}                      & 2021       &  T5-3B       &  Presents Creak, a dataset for commonsense  reasoning on entity knowledge   & Accuracy       & \ding{51}            \\  \cmidrule(l){3-8} 
                           &   &   \cite{wang2024causalbench}                      & 2024       & BERT-large, RoBERTa-large, DeBERTa-v3-large, DistillBERT-mnli, LLAMA models, OPT models, InternLM models, Falcon models, GPT-3.5-Turbo, GPT-4, GPT-4-Turbo     &  Proposes CausalBench benchmark for measuring LLMs’ causal learning capability     &  F1 score, structural hamming distance, structural intervention distance        & \ding{55}            \\ 
                           
                           \cmidrule(l){3-8}

			 &   &   \cite{hua2024disentangling}                      & 2024       & Qwen, LLaMA, GPT-3.5    &  Presents ContextHub to assess LLMs' reasoning across abstract and contextual tasks     & Average F1 score          & \ding{51}            \\  \cmidrule(l){3-8} 

                            &   &   \cite{cobbe2021training}                      & 2021      &  GPT-3      &    Designs GSM8K, a dataset of grade school math word problems, that evaluates LLMs’ mathematical reasoning capabilities        & Test solve rate      & \ding{55}            \\  \cmidrule(l){3-8} 

 &   &   \cite{suzgun2022challenging}                      & 2022       &  PaLM, Codex (code-davinci-002)       &  Showcases that CoT prompting significantly enhances LLMs’ performance on the challenging BIG-Bench Hard tasks  &   Exact match           & \ding{51}            \\  \cmidrule(l){2-8} 

                            
                          & Learning              
                          &   \cite{chang2023learning}& 2023& GPT-4, Claude2, LLama2 & Using CommonGen tasks to measure the learning ability of LLMs & BLEU, CIDEr-D, SPICE& \ding{51}       
                          \\ \cmidrule(l){3-8}
                          
                          &&   \cite{an2023learning}& 2023& GPT-4, LLaMA, LLaMA2, WizardMath, MetaMath, CodeLLaMA & LLMs' learning abilities are tested using datasets, such as GSM8K, MATH, SVAMP, ASDiv, CSQA, etc.& Accuracy & \ding{51}       
                          \\ \cmidrule(l){3-8}  

                          &&   \cite{jovanovic2024towards}& 2024& BERT, GPT4.0 & LLMs' learning abilities are tested using datasets, such as CIFAR-100, ImageNet100, etc.& Accuracy & \ding{51}       
                          \\ \cmidrule(l){3-8}  

                          &&   \cite{ren2024learning}& 2024& Pythia-410M/1B/1.4B/2.8B, T5-small, T5-large, LLaMA-2-13B, LLaMA-70B, RoBERTa & LLMs' learning abilities are tested using datasets such as Antropic HH and UltraFeedback.& Alignment performance, Generalization ability, Squeezing Effect & \ding{55}       
                          \\\midrule
                          
\multirow{2}{*}{Perceptual Skills}  
                          & Pattern Recognition    
                          & \cite{karamcheti2023language}& 2023 & GPT-3.5 & Introduces a framework for language-driven visual representation learning for robotics. & Various metrics across five robotics tasks & \ding{55}
                          \\ \cmidrule(l){3-8}
                           && \cite{qi2024shapellm}& 2024 & LLaMA & Presents a 3D multimodal LLM designed for embodied interaction, achieving state-of-the-art performance in 3D geometry understanding and language-unified interaction tasks. & Fine-tuned accuracy, zero-shot accuracy on various benchmarks & \ding{55}
                          \\ \cmidrule(l){3-8}
                           && \cite{hong20233d}& 2023 & GPT-4 & Proposes 3D-LLMs that incorporate the 3D physical world into LLMs, enabling models to perform 3D captioning, task decomposition, and spatially grounded dialogue. & BLEU-1, CIDER, accuracy on 3D question answering benchmarks & \ding{51} 
                          \\ \cmidrule(l){2-8}
                          
                          & Spatial Awareness      
                          &\cite{tan2024towards}& 2024 & GPT-4o & Proposes CRADLE, a multimodal agent framework for general computer control, capable of operating diverse software and completing complex tasks in video games. & Success rate across different software and games & \ding{51}  
                          \\ \cmidrule(l){3-8}
                          &&\cite{wang2023robogen}& 2024 & GPT-4 & Presents a generative robotic agent that learns diverse robotic skills via generative simulation, automating the learning process with minimal human supervision. & Skill diversity, success rate in simulations & \ding{55} 
                          \\ \cmidrule(l){3-8}        
                          &&\cite{schumann2024velma} & 2024 & GPT-4, CLIP & Introduces an embodied LLM agent for vision and language navigation in Street View, achieving 25\% improvement in task completion over state-of-the-art baselines. & Task completion rate in VLN & \ding{51}
                        \\ \midrule
\multirow{2}{*}{Analytical Skills}  
                          & Data Interpretation      
                          &\cite{hong2024data} & 2024 & GPT-4 & Introduces Data Interpreter, an LLM-based agent designed for data science, which integrates dynamic planning, tool utilization, and logical verification to enhance performance on data-centric tasks. & Machine learning accuracy, MATH dataset accuracy, open-ended task success & \ding{51}
                          \\ \cmidrule(l){3-8}
                          &&\cite{boiko2023autonomous}& 2023 & GPT-4 & Develops Coscientist, an AI system capable of autonomously designing, planning, and performing chemical experiments, demonstrating advanced capabilities in automated chemical research. & Task success rate in experimental synthesis, optimization tasks & \ding{55} 
                          \\ \cmidrule(l){3-8}
                          &&\cite{polak2024extracting}& 2024 & GPT-4 & Proposes ChatExtract, a conversational LLM-based method for automated data extraction from materials science literature, achieving high precision and recall via prompt engineering and redundancy. & Precision, recall for data extraction & \ding{55}         
                          \\ \cmidrule(l){2-8}
                          
                          & Information Processing       &    \cite{zhang2023large}      &   2023    &  GPT-3, BART  &  Introduces RPT (Relational Pre-trained Transformer), a Transformer-based denoising autoencoder that generalizes BERT and GPT architectures to automate data preparation tasks &  F1 &        \ding{55}  \\

                           \cmidrule(l){3-8}
                           &       &    \cite{borisov2022language}      &   2022    &  GPT-2  &  Presents GReaT, a method that utilizes auto-regressive LLMs to generate highly realistic synthetic tabular data &  	Machine learning efficiency, distance to closest records histogram, discriminator measure, bivariate joint distribution plots, ROCAUC score, F1 score &      \ding{55}  \\

                             \cmidrule(l){3-8}          
                             &       &    \cite{zou2024docbench}      &   2024    &  
GPT-3.5, GPT-4, GPT-4o, GLM-4, ChatGLM3, KimiChat, Mistral, LLaMA-2, LLaMA-3, InternLM2, Yi-1.5, Phi-3, Gemma, Command-R, Claude-3, Qwen-2.5, ERNIE-3.5
  &  Designs DOCBENCH, a comprehensive benchmark designed to evaluate LLM-based document reading systems &  Accuracy &        \ding{51} \\
                             \cmidrule(l){3-8}          


&       &    \cite{dai2024cocktail}      &   2024    &  BERT, RoBERTa, DistilBERT, MiniLM, T5  &  Proposes Cocktail, a benchmark of 16 datasets integrating human-written and LLM-generated content to evaluate information retrieval models in mixed-source data &  Retrieval accuracy  &       \ding{51} \\
                             \cmidrule(l){2-8}          


                          & Creativity     
                          &\cite{girotra2023ideas}           &2023       &GPT-4     &ChatGPT-4 outperforms students in creative generation, with high output and quality of ideas.  &Accuracy, Consistency, Relevance  &  \ding{51}
                          \\ \cmidrule(l){3-8}
                           &&\cite{xu2024jamplate}& 2024 & GPT-4&Introduced Jamplate system design to enhance LLM's creative reflection ability. & Accuracy & \ding{55}         
                          \\ \cmidrule(l){3-8}
                          &&\cite{li2024map}& 2024 & GPT, BERT&New mapping method for human LLM interaction mode. & Human-AI Collaboration Dimension, Implement-Creation Dimension. & \ding{55}         
                          \\ \cmidrule(l){3-8}
                          &&\cite{lu2024llm}& 2024 & GPT-4, GPT-3.5-turbo&Propose a framework and role-playing techniques to enhance LLM creativity, and use Alternative Uses Task to evaluate the creativity of LLM. & Fluency, Flexibility & \ding{51}         
                                \\ \midrule
\multirow{2}{*}{Executive Functioning}  
                          & Adaptability and Flexibility      &           &       & &  &  &            \\ \cmidrule(l){2-7}
                          & Planning and Organization       
                          & \cite{song2023llm}          &2023       &GPT-3  &The ALFRED dataset was used to evaluate the planning and organizational capabilities of LLM.  &Success Rate, Goal-Condition Success Rate &\ding{55}
                          \\ \cmidrule(l){3-8}
                          && \cite{kambhampati2024llms}          &2024       &GPT-4, GPT-3.5  &PlanBench benchmark was used to evaluate LLM's planning and organizational capabilities.  &Success Rate, Correctness Rate, Plan Pass Rates &\ding{55}
                          \\ \cmidrule(l){3-8}
                          && \cite{gundawar2024robust}          &2024       &GPT-4 Turbo, GPT-3.5 Turbo  &Use the Travel Planning Benchmark to evaluate LLM's planning and organizational capabilities.  &Delivery Rate, Final Pass Rate &\ding{51}
                          \\ \cmidrule(l){3-8}
                          && \cite{sharan2023llm}          &2023       &GPT-4, Llama2, GPT-3  &Use nuPlan Benchmark to evaluate LLM's planning and organizational capabilities.  &Score, Drivable &\ding{55}
                          \\ \cmidrule(l){2-8}
                          
&  Decision-Making  &    \cite{huang2024far}      &   2024    &  GPT-3.5, GPT-4, Gemini-Pro, LLaMA-3.1, Mixtral, Qwen-2  &  Introduces GAMA(γ)-Bench, a framework for evaluating LLM's decision-making abilities in multi-agent environments
 & Nash equilibrium 
 &        \ding{51}

\\ \cmidrule(l){3-8}

% &    &    \cite{pilditch2024reasoning}      &   2024    &  GPT models  &  Examines the risks associated with relying on LLMs, for reasoning under uncertainty, highlighting their limitations compared to human performance and proposing solutions to mitigate misuse &  	Accuracy, robustness, brier scores, coherence-based frameworks, decision quality metrics  &      \ding{51}

% \\ \cmidrule(l){3-8}


&    &    \cite{schramowski2022large}      &   2022    &  BERT, GPT-2, GPT-3  &  Assesses the risks of relying on LLMs for reasoning under uncertainty
 &  Toxicity probability, expected maximum toxicity
 &         \ding{51}


\\ \cmidrule(l){3-8}

&    &    \cite{echterhoff2024cognitive}      &   2024    &  GPT-3.5-turbo, GPT-4, Llama-2 models  &  Presents BIASBUSTER, a framework that evaluates and mitigates cognitive biases in LLM-assisted decision-making tasks
  &  Euclidean distance &        \ding{51}
      
                                \\ \midrule
\multirow{2}{*}{Social Skills} 
                          & Interpersonal Communication  
                          & \cite{park2023generative} & 2023 & ChatGPT & Proposes generative agents as believable simulacra of human behavior, implementing them in a sandbox game environment to simulate social interactions, forming relationships, and executing plans autonomously. & Observational consistency and emergent behavior analysis & \ding{55}
                          \\ \cmidrule(l){3-8}
                          && \cite{shanahan2023role}& 2023 & GPT-4, LLaMA & Introduces a conceptual framework for understanding LLM-based dialogue agents as role-playing entities, emphasizing metaphorical approaches to avoid anthropomorphism in agent design. & Qualitative analysis of role-play interactions & \ding{55} 
                          \\ \cmidrule(l){3-8}
                          &&\cite{strachan2024testing}& 2024 & GPT-4, GPT-3.5, LLaMA2-70B & Examines the capability of LLMs to exhibit theory of mind by testing them on a comprehensive set of psychological tasks, showing mixed performance across tasks like false beliefs, irony, and faux pas. & Performance accuracy on theory of mind tests & \ding{51}          
                          \\ \cmidrule(l){2-8}
                          
                          & Emotional Intelligence 
                          & \cite{sabour2024emobench} & 2024 & GPT-4, Baichuan, ChatGLM-3 & Proposes EMOBENCH, a comprehensive benchmark for evaluating Emotional Intelligence (EI) of LLMs, emphasizing gaps between LLMs and humans in understanding emotions. & Accuracy in emotional understanding tasks & \ding{51} 
                          \\ \cmidrule(l){3-8}
                          &&\cite{zhao2024both}& 2024 & Flan-T5, LLaMA-2-Chat & Introduces EIBENCH, a collection of EI-related tasks, and proposes MoEI, a modular EI enhancement method to improve LLMs' EI without compromising their General Intelligence (GI). & Accuracy on EI and GI benchmarks & \ding{55}
                          \\ \cmidrule(l){3-8}
                          &&\cite{wang2023emotional} & 2024 & GPT-4, Claude, LLaMA-based models & Presents SECEU, a psychometric evaluation of Emotional Understanding (EU) for LLMs, showing that GPT-4 achieves higher emotional intelligence scores than 89\% of human participants. & Standardized EQ scores, comparison to human performance & \ding{51}
                          \\ \cmidrule(l){2-8} 
                          

                          & Collaboration &    \cite{liu2023dynamic}      &   2023    &  GPT-3.5-Turbo, GPT-4  & Introduces DyLAN (Dynamic LLM-Agent Network), a framework that optimizes LLM-agent collaboration through dynamic agent selection, enhancing efficiency and adaptability in complex tasks &  Accuracy, \#API  &         \ding{55}            \\ \cmidrule(l){3-8}


&   &    \cite{chen2024llmarena}      &   2024    &  GPT-4, GPT-3.5, Qwen, LLaMA-2, AgentLM, DeepSeek, SUS, Yi, WizardLM, Vicuna  &  Presents LLMARENA, a benchmark designed to evaluate the abilities of LLMs in multi-agent, dynamic settings across seven different gaming environments
 &  TrueSkill™, reward &        \ding{51}            \\ \cmidrule(l){3-8}

&    &    \cite{zhang2024towards}      &   2024    &  GPT-4, GPT-3.5-Turbo, Qwen, LLaMA-2, AgentLM, and DeepSeek &  Proposes ReAd (Reinforced Advantage), a closed-loop feedback mechanism for LLM planners to enhance decision-making and efficiency in multi-agent collaboration
 &  Success rate, environment steps, number of queries &         \ding{55}            \\ \cmidrule(l){3-8}



&    &    \cite{piatti2024cooperate}      &   2024    & GPT-3.5, GPT-4, GPT-4o, Claude-3, LlaMA-2, LlaMA-3, Mistral, Qwen  &  Introduces GOVSIM, a generative simulation benchmark designed to evaluate the cooperative decision-making abilities of LLM-based agents in multi-agent resource-sharing scenarios &  Survival rate and time, total gain, efficiency, Equality, Over-usage &        \ding{55}            \\ 
                        \cmidrule(l){2-8}


                          &    &    \cite{dudy2024analyzing}      &   2024    &  Mistral, Gemma, Llama-2, GPT-3.5-Turbo, GPT-4-Turbo-Preview &  Evaluates how LLMs represent emotions across different cultures, particularly in mixed-emotion scenarios
 &  T-Test &         \ding{51}            \\ \cmidrule(l){3-8}

%&    &    \cite{chang2024benchmarking}      &   2024    &  GPT-4o, Gemini 1.5 Pro, Claude 3.5 Sonnet, LLaMA 3.1, with RAG  &  Presents a benchmark to evaluate LLMs in understanding and processing Hakka cultural knowledge
 &  Accuracy &         \ding{55}            \\ \cmidrule(l){3-8}



&    &    \cite{kharchenko2024well}      &   2024    &  GPT-4, GPT-4o, LLaMA 3, Command R+, Gemma  &  Evaluates LLMs ability to understand and reflect cultural values based on Hofstede's Cultural Dimensions framework &  Pearson correlation coefficient, accuracy 
 &         \ding{55}            \\ \cmidrule(l){3-8}




&    &    \cite{myung2024blend}      &   2024    &  The paper evaluates 16 LLMs, including GPT-4, GPT-3.5, Claude-3-Opus, Claude-3-Sonnet, Claude-3-Haiku, PaLM2, Gemini-1.0-Pro, C4AI Command R+, C4AI Command R, Qwen-1.5, SeaLLM, HyperCLOVA-X, Aya-23, Aya-101  &  Designs BLEND benchmark to evaluate LLMs on their cultural knowledge of everyday life across diverse regions and languages
 &  Cultural knowledge, short-answer questions, multiple-choice questions, performance gap, local languages, English performance, cultural sensitivity &         \ding{51}            \\  
                          \\ \bottomrule
\label{table:paper_summary}
\end{tabular}
}
\end{table}





% \begin{table}[ht]
% \caption{Summary of LLM competencies by specific skill.}
% \scriptsize 
% \resizebox{\textwidth}{!}{%

% \begin{tabular}{p{2.3cm}p{2.1cm}p{8.8cm}}
% \toprule
% \textbf{Category} & \textbf{Skill} & \textbf{LLM Competency} \\ \midrule

% \multirow{3}{*}{\textbf{Cognitive Skills}} 
%     & Reasoning 
%     & LLMs excel in simpler tasks like structured, rule-based, and abstract logic as models become more advanced, but they struggle with more complex challenges such as multi-step reasoning, handling multiple premises, and adapting to contextual or generalization-based reasoning. \\
%     \cmidrule(lr){2-3}
%     & Learning & LLMs excel in generalization and feedback-based adaptation but lack traditional online learning and real-time parameter updates.  \\
%     \cmidrule(lr){2-3}
%     & Memory & LLMs excel in context retention and task adaptation but lack persistent memory and real-time recall of past interactions.  \\
%     \midrule

% \multirow{3}{*}{\textbf{Perceptual Skills}} 
%     & Pattern Recognition & Achieved state-of-the-art performance in 3D shape understanding, approaching human-level performance \\
%     \cmidrule(lr){2-3}
    
%     & Spatial Awareness & LLM falls short of human-level precision in some virtual environments \\
%     % \cmidrule(lr){2-3}
%     % & Spatial Navigation & Approaches human-level navigation efficiency in navigation tasks \\
%     \midrule

% \multirow{3}{*}{\textbf{Analytical Skills}} 
%     % & Literature Search & Outperforms traditional search engines \\
%     % \cmidrule(lr){2-3}
%     & Data Interpretation & Limited compared to human performance in entity recognition and relation extraction \\
%     \cmidrule(lr){2-3}
%     & Creativity & LLMs excel in rapid, high-quality idea generation but lack human-like intuition, emotional depth, and true creative originality.  \\
%     \cmidrule(lr){2-3}
%     & Information Processing & LLMs excel in data integration, synthesis, and filtering, outperforming traditional deep neural networks with their natural language understanding, but they still lag behind humans in contextual and domain-specific comprehension. \\
%     \midrule

% \multirow{3}{*}{\textbf{Executive Functioning}} 
%     & Contextual Adaptation &  LLMs demonstrate improving contextual adaptation, excelling in structured tasks with real-time adjustments, but they still fall short of human flexibility and decision-making in unpredictable environments.\\
%     \cmidrule(lr){2-3}
%     & Planning and Organization & LLMs excel in generating and adapting plans but require external validation for reliability and logical consistency in complex tasks.  \\
%     \cmidrule(lr){2-3}
%     & Adaptability & LLMs excel in flexible decision-making and abstract reasoning but remain vulnerable to manipulation and harmful content extraction.  \\
%     \cmidrule(lr){2-3}
%     & Decision-Making & LLMs show considerable competency in decision-making, particularly in risk assessment and managing uncertainty, yet they struggle with cognitive biases inherent in their training data and require more robust mechanisms for responsible use in high-stakes and uncertain situations.\\
%     \midrule

% \multirow{2}{*}{\textbf{Emotional Skills}} 
   
%     % \cmidrule(lr){2-3}
%     % & Social Interaction & Demonstrates performance at or above human levels in false beliefs and irony detection, struggles with faux pas recognition \\
%     % \cmidrule(lr){2-3}
%     % & Communication & Performs at or above human levels in false beliefs and irony detection \\
%     \midrule
    
% \multirow{3}{*}{\textbf{Social Skills}} 
%     & Interpersonal communication & LLMs demonstrate significant progress in simulating human-like social interactions, excelling in structured scenarios and Theory of Mind tasks, but they still struggle with the depth and adaptability required for nuanced, real-world social dynamics.\\
%     \cmidrule(lr){2-3}
%     & Emotional Intelligence & Outperforms human participants in identifying and interpreting emotions \\
%     & Collaboration & LLMs showcase advances in collaboration and teamwork, but they continue to face challenges in matching the adaptability, strategic flexibility, and contextual awareness of human teams, particularly in complex and dynamic situations.\\
%     \cmidrule(lr){2-3}
%     & Cultural Competency & LLMs show promise in understanding and simulating cultural behaviors, especially in recalling factual knowledge, but they struggle with nuanced cultural sensitivity, particularly for underrepresented cultures, where humans consistently outperform them in adapting responses based on complex cultural contexts.\\

% \bottomrule
% \end{tabular}%
% }
% \end{table}

% \begin{table}[[!htpb]
%     \scriptsize 
%     \begin{longtable}{L{2.8cm}L{2.5cm}L{7cm}}
%         \caption{Summary of benchmarks for evaluating LLM's skills.} \\
%         \toprule
%         \textbf{Category} & \textbf{Skill} & \textbf{Benchmarks} \\
%         \midrule
%         \endfirsthead
    
%         \toprule
%         \textbf{Category} & \textbf{Skill} & \textbf{Benchmarks} \\
%         \midrule
%         \endhead
    
%         \bottomrule
%         \endlastfoot
    
%         \multirow{3}{=}{\textbf{Cognitive Skills}} 
    
%          & \multirow{1}{=}{Reasoning} 
%         & Deductive reasoning: LogiQA 2.0~\cite{liu2023logiqa}, PrOntoQA~\cite{saparov2022language}\\ 
%         \cmidrule(lr){3-3}
%         && Inductive reasoning: CommonsenseQA 2.0~\cite{talmor2022commonsenseqa}, StrategyQA~\cite{geva2021did}, Creak~\cite{onoe2021creak} \\ 
%         \cmidrule(lr){3-3}
%         && Causal reasoning: CausalBench~\cite{wang2024causalbench}, ContextHub~\cite{hua2024disentangling} \\ 
%         \cmidrule(lr){3-3}
%         && Mathematical reasoning: GSM8K~\cite{cobbe2021training} \\ 
%         \cmidrule(lr){3-3}
%         && General reasoning: BIG-Bench-Hard~\cite{suzgun2022challenging} \\ 
%         \cmidrule(lr){2-3}
    
%         & Learning & CommonGen~\cite{chang2023learning} \\
%         \cmidrule(lr){2-3}
%         & Memory & Visual Language Navigation (VLN-CE)~\cite{zhang2023memory} \\
%         \midrule
        
%         \multirow{2}{=}{\textbf{Perceptual Skills}} 
%         & Pattern Recognition & ScanQA~\cite{hong20233d} \\
%         \cmidrule(lr){2-3}
%         & Spatial Awareness & Red Dead Redemption 2 (RDR2)~\cite{tan2024towards}, MP3D (Matterport3D)~\cite{zhou2023esc}\\
%         \midrule
    
%         \multirow{3}{=}{\textbf{Analytical Skills}} 
%         & Data Interpretation & Metal-Organic Frameworks (MOFs) Information Extraction~\cite{dagdelen2024structured}, CORD-19 Challenge and Direction Extraction~\cite{lahav2022search} \\
%         \cmidrule(lr){2-3}
%         & Creativity & Purchase Intent Scores~\cite{xu2024jamplate} \\
%         \cmidrule(lr){2-3}
%         & \multirow{2}{=}{Information Processing} & DOCBENCH~\cite{zou2024docbench} \\ \cmidrule(lr){3-3} & & Cocktail~\cite{dai2024cocktail} \\ 
%         \midrule
    
%         \multirow{3}{=}{\textbf{Executive Functioning}} 
%         & Contextual Adaptation & LLM-CI~\cite{shvartzshnaider2024llm} \\
%         \cmidrule(lr){2-3}
        
%         & Planning and Organization & Embodied Agent Tasks~\cite{song2023llm} \\
%         \cmidrule(lr){2-3}
%         & Decision-Making & $\gamma$-Bench~\cite{huang2024far} \\
%         \midrule
    
%         \multirow{1}{=}{\textbf{Emotional Skills}} 
%         & Emotional Intelligence & LEAS (Levels of Emotional Awareness Scale)~\cite{elyoseph2023chatgpt} \\ 
%         \midrule
        
%         \multirow{3}{=}{\textbf{Social Skills}} 
%         & Social Interaction & False Belief Task~\cite{strachan2024testing}, Communication, Book Genre Typicality (Mystery and Romance)~\cite{le2023uncovering}  \\
%         \cmidrule(lr){2-3}
%         & Collaboration and Teamwork & LLMARENA~\cite{chen2024llmarena} \\
    
%         \cmidrule(lr){2-3}
%         & Cultural Competency & BLEND~\cite{myung2024blend}, Hofstede's Cultural Dimensions (HCD)~\cite{bhatt2024extrinsic} \\
%         % \midrule
%         % \multirow{2}{=}{\textbf{Moral and Ethical Skills}} 
%         % & Trustworthiness and Transparency & Domain-Specific Knowledge Graphs~\cite{lipizzi2024tell} \\
%         \bottomrule
%         % \multirow{1}{=}{\textbf{Collaboration and Teamwork}} 
%     \end{longtable}
% \end{table}




% \begin{longtable}{L{2.5cm}L{3.1cm}L{6cm}}
%     \caption{Summary of LLM competencies by specific skill.} \\
%     \toprule
%     \textbf{Category} & \textbf{Skill} & \textbf{LLM Competency} \\
%     \midrule
%     \endfirsthead

%     \toprule
%     \textbf{Category} & \textbf{Skill} & \textbf{LLM Competency} \\
%     \midrule
%     \endhead

%     \bottomrule
%     \endlastfoot

%     \multirow{2}{=}{\textbf{Cognitive Skills}} 
%     & Reasoning 
%     & LLMs excel in simpler tasks like structured, rule-based, and abstract logic as models become more advanced, but they struggle with more complex challenges such as multi-step reasoning, handling multiple premises, and adapting to contextual or generalization-based reasoning.\\
%     \cmidrule(lr){2-3}
%     & Learning & LLMs excel in generalization and feedback-based adaptation but lack traditional online learning and real-time parameter updates.  \\
%     \cmidrule(lr){2-3}
%     & Memory & LLMs excel in context retention and task adaptation but lack persistent memory and real-time recall of past interactions.  \\
%     \midrule
%     % \multirow{1}{=}{\textbf{Reasoning Skills}} 
%     % & Reasoning 
%     % & LLMs excel in simpler tasks like structured, rule-based, and abstract logic as models become more advanced, but they struggle with more complex challenges such as multi-step reasoning, handling multiple premises, and adapting to contextual or generalization-based reasoning.\\

    
%     \multirow{3}{=}{\textbf{Perceptual Skills}} 
%     & Environmental Perception & LLM falls short of human-level precision in some virtual environments \\
%     \cmidrule(lr){2-3}
%     & Pattern Recognition & Achieved state-of-the-art performance in 3D shape understanding, approaching human-level performance \\
%     \cmidrule(lr){2-3}
%     & Spatial Navigation & Approaches human-level navigation efficiency in navigation tasks \\
%     \midrule

%     \multirow{3}{=}{\textbf{Emotional and Social Skills}} 
%     & Emotional Intelligence & Outperforms human participants in identifying and interpreting emotions \\
%     \cmidrule(lr){2-3}
%     & Social Interaction & Demonstrates performance at or above human levels in false beliefs and irony detection, struggles with faux pas recognition \\
%     \cmidrule(lr){2-3}
%     & Communication & Performs at or above human levels in false beliefs and irony detection \\
%     \midrule

%     \multirow{4}{=}{\textbf{Analytical Skills}} 
%     & Literature Search & Outperforms traditional search engines \\
%     \cmidrule(lr){2-3}
%     & Data Interpretation & Limited compared to human performance in entity recognition and relation extraction \\
%     \cmidrule(lr){2-3}
%     & Creativity & LLMs excel in rapid, high-quality idea generation but lack human-like intuition, emotional depth, and true creative originality.  \\
%     \cmidrule(lr){2-3}
%     & Information Processing & LLMs excel in data integration, synthesis, and filtering, outperforming traditional deep neural networks with their natural language understanding, but they still lag behind humans in contextual and domain-specific comprehension. \\
%     \midrule

%     \multirow{3}{=}{\textbf{Executive Functioning}} 
%     & Planning and Organization & LLMs excel in generating and adapting plans but require external validation for reliability and logical consistency in complex tasks.  \\
%     \cmidrule(lr){2-3}
%     & Adaptability & LLMs excel in flexible decision-making and abstract reasoning but remain vulnerable to manipulation and harmful content extraction.  \\
%     \cmidrule(lr){2-3}
%     & Decision-Making & LLMs show considerable competency in decision-making, particularly in risk assessment and managing uncertainty, yet they struggle with cognitive biases inherent in their training data and require more robust mechanisms for responsible use in high-stakes and uncertain situations.\\
%     \midrule

%     \multirow{2}{=}{\textbf{Cultural and Contextual Competency}} 
%     & Cultural Competency & LLMs show promise in understanding and simulating cultural behaviors, especially in recalling factual knowledge, but they struggle with nuanced cultural sensitivity, particularly for underrepresented cultures, where humans consistently outperform them in adapting responses based on complex cultural contexts.
% \\
%     \cmidrule(lr){2-3}
%     & Contextual Competency &  LLMs demonstrate improving contextual adaptation, excelling in structured tasks with real-time adjustments, but they still fall short of human flexibility and decision-making in unpredictable environments.
% \\
%     \midrule

%     \multirow{4}{=}{\textbf{Moral and Ethical Skills}} 
%     & Trustworthiness and Transparency & LLMs show potential in credibility and transparency, but challenges remain in explainability, ethical consistency, and mitigating biases.  \\ 
%     \midrule

%     \multirow{1}{=}{\textbf{Collaboration and Teamwork}} 
%      & Collaboration and Teamwork & LLMs showcase promise in collaboration and teamwork, but they continue to face challenges in matching the adaptability, strategic flexibility, and contextual awareness of human teams, particularly in complex and dynamic situations.\\
    
% \end{longtable}

% \begin{table}[]
% \caption{Summary of benchmarks for evaluating LLM's skills.} 
% \scriptsize 
% \resizebox{\textwidth}{!}{%
% \begin{longtable}{p{2.3cm}p{2.3cm}p{2.5cm}p{6cm}}
%     \toprule
%     \textbf{Category} & \textbf{Skill} & \textbf{Benchmarks} & \textbf{Description} \\
%     \midrule
%     \endfirsthead

%     \toprule
%     \textbf{Category} & \textbf{Skill} & \textbf{Benchmarks} & \textbf{Description} \\
%     \midrule
%     \endhead

%     \bottomrule
%     \endlastfoot

%     \multirow{4}{=}{\textbf{Cognitive Skills}} 
%     & \multirow{5}{=}{Reasoning} 
%     & Deductive reasoning: LogiQA 2.0~\cite{liu2023logiqa}, PrOntoQA~\cite{saparov2022language} 
%     & LogiQA 2.0 focuses on categorical, disjunctive, and conditional reasoning. PrOntoQA involves deriving specific conclusions from logical premises using first-order logic. \\ 
%     \cmidrule(lr){3-4}
%     && Inductive reasoning: CommonsenseQA 2.0~\cite{talmor2022commonsenseqa}, StrategyQA~\cite{geva2021did}, Creak~\cite{onoe2021creak} 
%     & CommonsenseQA 2.0 tests generalization from everyday knowledge. StrategyQA challenges models to infer general principles from specific questions. Creak evaluates models' ability to identify logical inconsistencies using commonsense knowledge. \\ 
%     \cmidrule(lr){3-4}
%     && Causal reasoning: CausalBench~\cite{wang2024causalbench}, ContextHub~\cite{hua2024disentangling} 
%     & CausalBench tests causal reasoning about cause-and-effect relationships. ContextHub evaluates causal reasoning in both abstract and contextual tasks. \\ 
%     \cmidrule(lr){3-4}
%     && Mathematical reasoning: GSM8K~\cite{cobbe2021training} 
%     & GSM8K evaluates complex mathematical problem-solving with deductive logic. \\ 
%     \cmidrule(lr){3-4}
%     && General reasoning: BIG-Bench-Hard~\cite{suzgun2022challenging} 
%     & BIG-Bench-Hard evaluates abstract, deductive, inductive, and commonsense reasoning tasks. \\ 
%     \midrule

%     & Learning & CommonGen\cite{chang2023learning} & Tests models on generating coherent sentences from unordered concept words, emphasizing commonsense reasoning. \\ 
%     \cmidrule(lr){2-4}
%     & Memory & VLN-CE~\cite{zhang2023memory} & A task where an agent navigates through a 3D environment based on natural language instructions, using visual perception and language understanding. \\ 
%     \midrule

%     \multirow{3}{=}{\textbf{Perceptual Skills}} 
%     & Environmental Perception & RDR2~\cite{tan2024towards} & A complex 3D role-playing game. The benchmark involves embodied navigation, interaction, and exploring virtual environments. \\ 
%     \cmidrule(lr){2-4}
%     & Pattern Recognition & ScanQA~\cite{hong20233d} & Focuses on spatial scene understanding and answering questions related to spatial relationships and object positions in 3D environments. \\ 
%     \cmidrule(lr){2-4}
%     & Spatial Navigation & MP3D~\cite{zhou2023esc} & Evaluates agents' ability to navigate realistic indoor environments and locate goal objects. \\ 
%     \midrule

%     \multirow{3}{=}{\textbf{Emotional and Social Skills}} 
%     & Emotional Intelligence & LEAS~\cite{elyoseph2023chatgpt} & A test for measuring emotional awareness through responses to emotionally charged scenarios. \\ 
%     \cmidrule(lr){2-4}
%     & Social Interaction & False Belief Task~\cite{strachan2024testing} & Evaluates understanding that others may hold beliefs that are false, a key test in theory of mind research. \\ 
%     \cmidrule(lr){2-4}
%     & Communication & Book Genre Typicality~\cite{le2023uncovering} & Evaluates how well GPT-4 assesses the typicality of books in specific literary genres. \\ 
%     \midrule

%     \multirow{4}{=}{\textbf{Analytical Skills}} 
%     & Literature Search & CORD-19 Challenge~\cite{lahav2022search} & Focuses on extracting scientific challenges and research directions from COVID-19-related research papers. \\ 
%     \cmidrule(lr){2-4}
%     & Data Interpretation & MOFs Information Extraction~\cite{dagdelen2024structured} & Extracts structured information from scientific texts, such as chemical formulae, applications, and descriptive data. \\ 
%     \cmidrule(lr){2-4}
%     & Creativity & Purchase Intent Scores~\cite{xu2024jamplate} & Measures consumer likelihood to buy a product or service, typically using scales to predict potential sales. \\ 
%     \cmidrule(lr){2-4}
%     & Information Processing & DOCBENCH~\cite{zou2024docbench} & Processes raw PDFs to evaluate tasks like file parsing and metadata extraction, highlighting gaps in LLMs' real-world document comprehension. \\ 
%     \midrule

%     \multirow{3}{=}{\textbf{Executive Functioning}} 
%     & Planning and Organization & Embodied Agent Tasks~\cite{song2023llm} & AI-driven agents navigate environments, testing perception, planning, and physical movement guided by visual or linguistic instructions. \\ 
%     \cmidrule(lr){2-4}
%     & Decision-Making & $\gamma$-Bench~\cite{huang2024far} & Uses multi-agent game theory scenarios to evaluate decision-making, including cooperative and betraying strategies. \\ 
%     \midrule

%     \multirow{2}{=}{\textbf{Cultural and Contextual Competency}} 
%     & Cultural Competency & BLEND~\cite{myung2024blend} & 52.6k question-answer pairs from 16 countries and 13 languages, evaluating cultural knowledge. \\ 
%     \cmidrule(lr){2-4}
%     & Contextual Competency & LLM-CI~\cite{shvartzshnaider2024llm} & Evaluates LLMs' ability to encode societal privacy norms across different contexts. \\ 
%     \midrule

%     \multirow{2}{=}{\textbf{Moral and Ethical Skills}} 
%     & Trustworthiness and Transparency & Domain-Specific Knowledge Graphs~\cite{lipizzi2024tell} & Structured representations of domain-specific information, such as medicine or finance, to help models understand and reason within specific fields. \\ 
%     \midrule

%     \multirow{1}{=}{\textbf{Collaboration and Teamwork}} 
%     & Collaboration and Teamwork & LLMARENA~\cite{chen2024llmarena} & Evaluates collaboration and decision-making in multi-agent environments through seven distinct gaming scenarios. \\ 
% \bottomrule
% \end{longtable}
% }
% \end{table}




% \iffalse
%  \begin{longtable}[ht]{L{2cm}L{2cm}L{2.3cm}L{5cm}}
%     \caption{Summary of benchmarks for evaluating LLM's skills.} \\
%     \toprule
%     \textbf{Category} & \textbf{Skill} & \textbf{Benchmarks} & \textbf{Description} \\
%     \midrule
%     \endfirsthead

%     \toprule
%     \textbf{Category} & \textbf{Skill} & \textbf{Benchmarks} & \textbf{Description} \\
%     \midrule
%     \endhead

%     \bottomrule
%     \endlastfoot

%     \multirow{4}{=}{\textbf{Cognitive Skills}} 

%      & \multirow{3}{=}{Reasoning} 
%     & Deductive reasoning: LogiQA 2.0~\cite{liu2023logiqa}, PrOntoQA~\cite{saparov2022language} 
%     & LogiQA 2.0 focuses on deductive reasoning involving categorical, disjunctive, and conditional reasoning types. PrOntoQA involves deductive reasoning tasks based on first-order logic, where models derive specific conclusions from premises. \\ 
%     \cmidrule(lr){3-4}
%     && Inductive reasoning: CommonsenseQA 2.0~\cite{talmor2022commonsenseqa}, StrategyQA~\cite{geva2021did}, Creak~\cite{onoe2021creak} 
%     & CommonsenseQA 2.0 tests inductive reasoning by requiring models to generalize from everyday knowledge. StrategyQA also tests inductive reasoning, challenging models to infer general principles from specific questions and knowledge. Creak evaluates inductive reasoning through the identification of logical inconsistencies using commonsense knowledge. \\ 

%     \cmidrule(lr){3-4}
%     && Causal reasoning: CausalBench~\cite{wang2024causalbench}, ContextHub~\cite{hua2024disentangling} 
%     & CausalBench tests causal reasoning, focusing on the ability to reason about cause-and-effect relationships across different domains. ContextHub also focuses on causal reasoning but in both abstract and contextualized tasks. \\ 

%     \cmidrule(lr){3-4}
%     && Mathematical reasoning: GSM8K~\cite{cobbe2021training} 
%     & GSM8K evaluates mathematical reasoning, where models solve complex mathematical problems through deductive logic and reasoning. \\ 

%     \cmidrule(lr){3-4}
%     && General reasoning: BIG-Bench-Hard~\cite{suzgun2022challenging} 
%     & BIG-Bench-Hard evaluates models on a mix of abstract, deductive, inductive, and commonsense reasoning tasks. \\ 
%     \midrule


%     % & \multirow{10}{=}{Reasoning} & LogiQA 2.0~\cite{liu2023logiqa} & Type: Deductive reasoning. 
    
%     % Focuses on five types of reasoning: categorical, sufficient conditional, necessary conditional, disjunctive, and conjunctive reasoning. \\ \cmidrule(lr){3-4} & & PrOntoQA~\cite{saparov2022language} & Type: Deductive reasoning. 
    
%     % Involves first-order logic tasks where LLMs derive specific conclusions from logical premises. \\ \cmidrule(lr){3-4} & & CommonsenseQA 2.0 \cite{talmor2022commonsenseqa}& Type: Inductive reasoning. Requires generalization from everyday facts and commonsense knowledge. \\ \cmidrule(lr){3-4} & & StrategyQA~\cite{geva2021did} & Type: Inductive reasoning. 
    
%     % Involves inferring general principles from specific questions and external knowledge. \\ \cmidrule(lr){3-4} & & Creak ~\cite{onoe2021creak}& Type: Inductive reasoning. Tests LLMs' ability to generalize from commonsense knowledge to identify inconsistencies. \\ \cmidrule(lr){3-4} & & CausalBench~\cite{wang2024causalbench} & Type: Causal reasoning. 
    
%     % Tests LLMs' ability to reason about cause-and-effect relationships across domains. \\ \cmidrule(lr){3-4} & & ContextHub ~\cite{hua2024disentangling}& Type: Causal reasoning. 
    
%     % Evaluates causal reasoning in abstract and contextualized tasks.\\ \cmidrule(lr){3-4} & & GSM8K ~\cite{cobbe2021training}& Type: Mathematical reasoning. 
    
%     % Focuses on complex mathematical problem solving with deductive elements. \\ \cmidrule(lr){3-4} & & BIG-Bench-Hard ~\cite{suzgun2022challenging}& Type: General reasoning. 
    
%     % Evaluates LLM performance across abstract, deductive, inductive, and commonsense reasoning. \\    \midrule

    
%     & Learning &CommonGen\cite{chang2023learning} & The CommonGen dataset tests models on generating coherent sentences from unordered concept words, emphasizing commonsense reasoning. It includes around 35,000 sentences covering everyday scenarios for text generation tasks.\\
%     \cmidrule(lr){2-4}
%     & Memory & Visual Language Navigation (VLN-CE)\cite{zhang2023memory} & A task where an agent navigates through a 3D environment based on natural language instructions, using both visual perception and language understanding to complete navigation goals in complex environments.\\
%     \midrule

%     % \multirow{10}{=}{\textbf{Reasoning Skills}} 
%     % & \multirow{2}{=} {Deductive Reasoning} 
%     % & LogiQA 2.0~\cite{liu2023logiqa} & Focuses on five types of reasoning: categorical, sufficient conditional, necessary conditional, disjunctive, and conjunctive reasoning. \\ 
%     % \cmidrule(lr){3-4} 
%     % & & PrOntoQA~\cite{saparov2022language} & Involves first-order logic tasks where LLMs derive specific conclusions from logical premises. \\ 
    
%     % \cmidrule(lr){2-4}
%     % & \multirow{3}{=} {Inductive Reasoning}  
%     % & CommonsenseQA 2.0~\cite{talmor2022commonsenseqa} & Requires generalization from everyday facts and commonsense knowledge. \\ 
%     % \cmidrule(lr){3-4} 
%     % & & StrategyQA~\cite{geva2021did} & Involves inferring general principles from specific questions and external knowledge. \\ 
%     % \cmidrule(lr){3-4} 
%     % & & Creak~\cite{onoe2021creak} & Tests LLMs' ability to generalize from commonsense knowledge to identify inconsistencies. \\ 
    
%     % \cmidrule(lr){2-4}
%     % & \multirow{2}{=} {Causal Reasoning} 
%     % & CausalBench~\cite{wang2024causalbench} & Tests LLMs' ability to reason about cause-and-effect relationships across domains. \\ 
%     % \cmidrule(lr){3-4} 
%     % & & ContextHub~\cite{hua2024disentangling} & Evaluates causal reasoning in abstract and contextualized tasks. \\ 
    
%     % \cmidrule(lr){2-4}
%     % & \multirow{2}{=} {Mathematical Reasoning}  
%     % & GSM8K~\cite{cobbe2021training} & Focuses on complex mathematical problem solving with deductive elements. \\ 
%     % \cmidrule(lr){2-4} 
%     % & \multirow{2}{=} {General Reasoning}  
%     % & BIG-Bench-Hard~\cite{suzgun2022challenging} & Evaluates LLM performance across abstract, deductive, inductive, and commonsense reasoning. \\ 
    
%     \multirow{3}{=}{\textbf{Perceptual Skills}} 
%     & Environmental Perception & Red Dead Redemption 2 (RDR2) \cite{tan2024towards} & A complex 3D role-playing game with a rich storyline. The benchmark involves tasks like 3D embodied navigation and interaction, exploring virtual environments, and following storylines.\\
%     \cmidrule(lr){2-4}
%     & Pattern Recognition & ScanQA \cite{hong20233d} & A 3D question answering benchmark that focuses on spatial scene understanding. It requires the model to answer questions related to 3D environments by reasoning about spatial relationships and object positions. The benchmark tests the ability to integrate 3D spatial information and language understanding.\\
%     \cmidrule(lr){2-4}
%     & Spatial Navigation & MP3D (Matterport3D) \cite{zhou2023esc} & A dataset commonly used for embodied AI tasks, particularly object navigation. It contains 2,195 validation episodes across 11 environments and 21 object categories. This benchmark evaluates the agent's ability to navigate in realistic indoor environments to locate specific goal objects.\\
%     \midrule

%     \multirow{3}{=}{\textbf{Emotional and Social Skills}} 
%     & Emotional Intelligence & LEAS (Levels of Emotional Awareness Scale) \cite{elyoseph2023chatgpt} & A performance-based test used to measure emotional awareness by analyzing responses to emotionally charged scenarios. The benchmark compares ChatGPT's ability to identify and describe emotions with that of human norms, highlighting ChatGPT's superior emotional awareness over time.\\ 
%     \cmidrule(lr){2-4} 
%     & Social Interaction & False Belief Task \cite{strachan2024testing} & A well-established test in theory of mind research. It evaluates the model's or human's ability to understand that other individuals may hold beliefs that are false and differ from reality. In this task, the participant predicts where a character will look for an object based on the character's false belief about its location.\\
%     \cmidrule(lr){2-4}
%     & Communication & Book Genre Typicality (Mystery and Romance) \cite{le2023uncovering} & This benchmark evaluates how well GPT-4 can assess the typicality of books in specific literary genres like Mystery and Romance. The model is asked to rate the typicality of a book's description in a genre, using a score from 0 to 100, where higher scores indicate a book more typical of the genre.\\
%     \midrule

%     \multirow{4}{=}{\textbf{Analytical Skills}} 
%     & Literature Search & CORD-19 Challenge and Direction Extraction \cite{lahav2022search} & This benchmark focuses on extracting scientific challenges and research directions from the CORD-19 corpus, a large dataset of COVID-19 related research papers. The task involves identifying sentences that mention research challenges (e.g., limitations or difficulties) and potential directions (e.g., suggestions for future research) in the literature.\\
%     \cmidrule(lr){2-4}
%     & Data Interpretation & Metal-Organic Frameworks (MOFs) Information Extraction \cite{dagdelen2024structured} & This benchmark focuses on extracting structured information from scientific texts related to MOFs. It involves identifying chemical formulae, applications, guest species, and descriptive information about MOFs from research paper abstracts. \\
%     \cmidrule(lr){2-4}
%     & Creativity & Purchase Intent Scores\cite{xu2024jamplate}  & It measure how likely consumers are to buy a product or service. They typically use a scale (e.g., "definitely won't buy" to "definitely will buy") to quantify interest and predict potential sales.  \\
%     \cmidrule(lr){2-4}
%     % & Information Processing & & \\
%     & \multirow{2}{=}{Information Processing} & DOCBENCH~\cite{zou2024docbench} &  It processes raw PDFs and related questions to evaluate LLMs on tasks like file parsing, metadata extraction, and long-context understanding, revealing notable gaps compared to human comprehension in diverse real-world documents. \\ \cmidrule(lr){3-4} & & Cocktail~\cite{dai2024cocktail} & A comprehensive benchmark with 16 datasets, tailored for information retrieval, assessing LLMs' performance in processing mixed human-written and LLM-generated content, while highlighting key challenges in maintaining accuracy and mitigating biases across diverse, multi-source environments.
%     \\ 

%     \midrule

%     \multirow{3}{=}{\textbf{Executive Functioning}} 
%     & Planning and Organization & Embodied Agent Tasks\cite{song2023llm}  & It involve AI-driven agents interacting with and navigating real or simulated environments. These tasks test agents on abilities like perception, planning, and physical movement to complete objectives, often guided by visual or linguistic instructions.  \\
%     \cmidrule(lr){2-4}
%     & Adaptability & & \\
%     \cmidrule(lr){2-4}
%     & Decision-Making & $\gamma$-Bench~\cite{huang2024far}& A benchmarking framework that uses a dataset of 8 classic multi-agent game theory scenarios, including cooperative, betraying, and sequential games, to evaluate LLMs' decision-making competency by measuring their robustness, strategy formation, and generalizability in dynamic, multi-agent environments.\\
%     \midrule

%     \multirow{2}{=}{\textbf{Cultural and Contextual Competency}} 
%     & \multirow{2}{=}{Cultural Competency}& BLEND ~\cite{myung2024blend} & A benchmark with 52.6k question-answer pairs from 16 countries and 13 languages, including low-resource languages like Amharic and Sundanese, evaluating LLMs' everyday cultural knowledge.\\
   
%     \cmidrule(lr){3-4} && 
% Hofstede’s Cultural Dimensions (HCD) ~\cite{bhatt2024extrinsic}& A benchmark that evaluates cultural competence by assessing models across six dimensions—Power Distance, Individualism vs. Collectivism, Masculinity vs. Femininity, Uncertainty Avoidance, Long-term vs. Short-term Orientation, and Indulgence vs. Restraint—to determine their ability to understand and adapt to cultural nuances.\\
%     \cmidrule(lr){2-4}
%     & Contextual Competency & LLM-CI ~\cite{shvartzshnaider2024llm} & A benchmark that evaluates LLMs' ability to maintain contextual integrity by using a multi-prompt factorial vignette methodology, assessing how well they encode societal privacy norms across various contexts with datasets like IoT and COPPA vignettes.\\
%     \midrule

%     \multirow{4}{=}{\textbf{Moral and Ethical Skills}} 
%     & Trustworthiness and Transparency & Domain-Specific Knowledge Graphs\cite{lipizzi2024tell}  & Domain-specific knowledge graphs are structured representations of information tailored to a particular domain. They capture entities, relationships, and facts specific to that field (e.g., medicine or finance), helping systems understand and reason about domain-related content. \\
%     \midrule

%     \multirow{1}{=}{\textbf{Collaboration and Teamwork}} 
%     & Collaboration and Teamwork & LLMARENA~\cite{chen2024llmarena}&
% A dynamic benchmark designed to evaluate LLMs' collaboration and decision-making abilities in multi-agent environments, assessing key skills such as spatial reasoning, strategic planning, communication, opponent modeling, and teamwork through seven distinct gaming scenarios, with a comprehensive scoring system that measures performance across these areas. \\
   

% \end{longtable}
% \fi



\subsection{Reasoning}


% In the domain of inductive reasoning, while GPT-4 has made significant improvements in rule application and rule induction, it still faces challenges in generalizing to larger problems and scenarios with minimal examples. Bowen \textit{et al.}\cite{bowen2024comprehensive} found that although GPT-4 achieves up to 99.5\% partial accuracy in rule application tasks, its ability to extend this performance to more complex problems or limited data scenarios remains constrained. Even with the use of Chain-of-Thought prompting, designed to guide step-by-step reasoning, both GPT-4 and Davinci exhibit difficulties in rule validation and integrating complex rules, revealing significant gaps in their logical consistency and deep rule comprehension. Davinci's performance, in particular, declines to 51\% accuracy in tasks that demand nuanced rule handling. Complementing these findings, Han \textit{et al.}\cite{han2024inductive} evaluated GPT-3.5 and GPT-4 on property induction tasks, highlighting that while GPT-4 more closely aligns with human reasoning patterns, it still struggles to fully capture premise non-monotonicity, a critical element of human cognitive processing.

% In the domain of inductive reasoning, despite GPT-4's improved performance in rule application and rule induction tasks, it still encounters difficulties in rule validation and integrating complex rules. Bowen \textit{et al.}~\cite{bowen2024comprehensive} find that GPT-4 achieves 99.5\% partial accuracy in polygon grouping tasks but struggles to generalize when dealing with larger problems or when minimal examples are provided. Even with the support of techniques like Chain-of-Thought prompting—which aims to guide the model through step-by-step problem-solving—LLMs like GPT-4 and Davinci still face significant challenges in applying, validating, and integrating rules, especially in tasks requiring deep rule comprehension and logical integration. This limitation highlights the gap in LLMs’ ability to handle more complex inductive reasoning scenarios effectively.

% Causal reasoning in LLMs like GPT-4 and Davinci is challenging, particularly in complex text-based and coding-related tasks~\cite{wang2024causalbench}. While they perform adequately in mathematical causal tasks, they often misinterpret causal structures in narratives or code, leading to hallucinations~\cite{wang2023can}. Models like GPT-4 initially perform well but struggle with flawed or conflicting arguments, raising concerns about their reasoning consistency and depth.



% Causal reasoning capabilities in LLMs like GPT-4 and Davinci present significant challenges, as they often require a deep understanding of cause-and-effect relationships across different contexts. While these models demonstrate reasonable proficiency in mathematical causal tasks, evaluations using the CausalBench benchmark reveal their considerable struggles with more complex text-based and coding-related causal problems~\cite{wang2024causalbench}. These tasks require LLMs to accurately interpret causal structures within narratives or code snippets, where simple data correlations are insufficient. Developing a robust understanding of these dynamics is crucial to avoid generating hallucinations—misleading or incorrect outputs that undermine the credibility of AI systems. Even though models like GPT-4 initially perform well in causal reasoning tasks, their capabilities frequently deteriorate when confronted with flawed or conflicting arguments, raising concerns about the consistency and depth of their reasoning processes in such complex scenarios~\cite{wang2023can}.

% To address the limitations in generalizing causal reasoning and handling complex scenarios, the ContextHub benchmark was introduced to comprehensively evaluate the reasoning abilities of LLMs, including models like GPT-4, PaLM, and LLaMA, in both abstract and contextualized logical problems~\cite{hua2024disentangling}. ContextHub specifically aims to tackle the issues these models face when transitioning from isolated logic tasks to reasoning in diverse, real-world contexts, where their performance often declines. Findings from ContextHub indicate that while these larger models excel in handling straightforward logic problems, they frequently struggle to generalize their reasoning skills when faced with more nuanced, context-driven scenarios that require deeper interpretative abilities. Complementary datasets like GSM8K target mathematical problem-solving with a focus on deductive reasoning elements, while BIG-Bench-Hard provides a thorough evaluation of multi-step reasoning, factual knowledge, and commonsense reasoning capabilities~\cite{cobbe2021training, suzgun2022challenging}. Together, these benchmarks offer critical insights into the strengths and limitations of models like GPT-4 and Davinci, highlighting areas where further advancements are necessary to improve their reasoning capabilities in more complex, context-rich domains.



% Logical reasoning, a core element of human cognition, is essential for daily functioning. It covers various types of reasoning, such as deductive, inductive, and causal reasoning, each contributing to how we process information and make decisions. Deductive reasoning applies general principles to obtain specific conclusions, while inductive reasoning draws generalizations from specific observations~\cite{goswami2010inductive}, and causal reasoning helps understand cause-and-effect relationships~\cite{eells2016rational,binz2023using}. 

% % The LogiQA 2.0 dataset, a large-scale logical reasoning resource adapted from the Chinese Civil Service Examination, features 15,708 instances and a new NLI task with 35,000 premise-hypothesis pairs~\cite{liu2023logiqa}. It provides a fine-grained evaluation of deductive reasoning types, such as categorical, conditional, and disjunctive reasoning, and includes professional translations to remove cultural-specific elements like idioms for better generalizability. Despite LLMs like GPT-3 achieving 68.65\% accuracy in natural language inference (NLI), results still fall significantly below the 90\% human benchmark, underscoring ongoing challenges in handling complex logical reasoning. 

% The LogiQA 2.0 dataset, adapted from the Chinese Civil Service Examination, includes 15,708 instances and a new natural language inference (NLI) task with 35,000 premise-hypothesis pairs~\cite{liu2023logiqa}. It evaluates five different types of deductive reasoning like categorical and conditional reasoning, with translations to remove cultural-specific elements. While GPT-3 achieves 68.65\% accuracy in NLI, this remains below the 90\% human benchmark, underscoring ongoing challenges in complex logical reasoning. LLMs like GPT-3.5, PaLM, and LLaMA excel at basic deductive reasoning but struggle with more complex problems requiring multiple logical steps or containing multiple premises simultaneously~\cite{saparov2024testing}. Similarly, models such as GPT-4 and Davinci face difficulties in inductive reasoning, particularly in applying, validating, and integrating rules, even with the support of few-shot examples and Chain-of-Thought prompts~\cite{bowen2024comprehensive}. In causal reasoning, benchmarks like CausalBench~\cite{wang2024causalbench} reveal that while LLMs perform well in mathematical reasoning, they struggle with text-based and coding-related causal tasks, suggesting a connection between stronger causal reasoning abilities and reduced hallucination rates. Although models like GPT-4 initially perform well, their reasoning falters when faced with flawed or conflicting arguments, raising concerns about their depth of reasoning and alignment~\cite{wang2023can}. 

% To further tackle these challenges, ContextHub was introduced as a benchmark to evaluate LLMs’ reasoning abilities on both abstract and contextualized logical problems~\cite{hua2024disentangling}. The findings show that while larger models perform well on abstract logic tasks, their generalization remains limited, and performance varies significantly depending on the contextual domain. Additionally, several reasoning benchmarks have been employed to assess LLMs' capabilities, including GSM8K for mathematical reasoning~\cite{cobbe2021training}, PrOntoQA for first-order logic~\cite{saparov2022language}, and commonsense reasoning datasets such as StrategyQA~\cite{geva2021did}, CommonsenseQA 2.0~\cite{talmor2022commonsenseqa}, and Creak~\cite{onoe2021creak}. BIG-Bench-Hard~\cite{suzgun2022challenging} were also used to evaluate LLMs' performance across various reasoning domains, including multi-step reasoning, deductive reasoning, factual and commensense reasoning, providing comprehensive insights into their strengths and limitations.



% -----
% Logical reasoning, an essential ability for daily functioning, involves several components, including deductive, inductive, abductive, analogical, and causal reasoning. Deductive reasoning involves the ability to apply general principles to reach specific conclusions~\cite{goswami2010inductive}. Inductive reasoning involves using specific observations to draw general conclusions~\cite{goswami2010inductive}. Abductive reasoning refers to XXXX. Analogical reasoning xxx. Causal reasoning is crucial for understanding cause-and-effect relationships and the fundamental principles that govern them~\cite{eells2016rational,binz2023using}.

% Studies on deductive reasoning illustrate that LLM models, e.g., GPT-3.5, PaLM, LLaMA, FLAN-T5 perform well on basic deductive reasoning tasks, yet encounter difficulties with more complex tasks that contain more extensive logical steps or multiple premises all at once, especially when tasks are not part of the training~\cite{saparov2024testing}. 

% Despite LLM being able to work through simple tasks, LLMs, e.g., GPT-4, GPT-3, Davinci,  experienced challenges in inductive reasoning tasks by applying, validating, and integrating rules, even when few-shot examples and Chain-of-Through prompts are supported~\cite{bowen2024comprehensive}.



% Recently, a causal benchmark called CausalBench was proposed to give a comprehensive evaluation of LLMs' causal reasoning includes various aspects, i.e., text, math, and coding~\cite{wang2024causalbench}. The benchmark covers over 60,000 tasks and 6 metrics to measure LLMs' performance in understanding and reasoning about causal relationships. Applying the benchmark, LLMs like GPT-4 excel in mathematical problems, yet struggle with text and coding problems, especially when required to provide reasons from multiple perspectives. In addition, there is a noticeable connection between stronger causal reasoning capabilities and lower hallucination rates, suggesting that a model’s ability to grasp causal relationships may impact its factual accuracy.


% While LLMs like GPT-4 demonstrate strong performance in complex reasoning tasks, there is still uncertainty about whether they truly comprehend and follow truth and logic. A study shows that although they can produce accurate solutions at first, they frequently struggle to maintain their reasoning when challenged by a large number of flawed arguments or examples, indicating potential issues with their alignment and reasoning depth~\cite{wang2023can}.

\subsection{information processing}
% \begin{itemize}
%     \item Data integration and synthesis
%     Traditional deep neural networks have shown excellent performance in the field of data analytics \cite{tang2020rpt} and management\cite{chai2020crowdchart}, but as the data size increases, the models usually face the problems of insufficient generalization ability and poor semantic understanding. LLM's demonstrated excellence in the field of natural language understanding and generation contributes to better integration and synthesis of data. With a well-designed prompt technique, Zhao \textit{et al.} \cite{zhang2023large} achieved good results in data detection, data interpolation. This indicates that LLM has a good integration and semantic understanding of data preprocessing. NL2Rigel \cite{huang2023interactive} is an interactive system that helps users synthesize and enhance tables from semi-structured text using natural language instructions. High-quality synthetic data as a solution to the lack of data. GReaT \cite{borisov2022language} exploits an auto-regressive generative LLM to sample synthetic and yet highly realistic tabular data. 
%     \item Information filtering and relevance determination
%     Unlike conventional recommender systems and search engines, which act as passive mediums for information filtering, LLMs establish the groundwork for active user engagement\cite{galitsky2024llm}. Eigner \textit{et al.}\cite{eigner2024determinants} conduct a comprehensive literature analysis, providing a structural overview and detailed analysis of determinants impacting decision-making with LLM support. With a dependency framework, LLM improves decision quality in human-AI collaboration, empowering both users and organizations, and designing more effective. 
% \end{itemize}


% LLMs exhibit several competencies in information processing, particularly in the areas of data integration, synthesis, and information filtering. These capabilities are supported by their advanced natural language understanding and generation, which allow them to handle and process data in ways that surpass traditional deep neural networks.

% In terms of data integration and synthesis, traditional deep neural networks have been highly effective in data analytics \cite{tang2020rpt} and management \cite{chai2020crowdchart}. However, as data scales up, these models often encounter limitations such as insufficient generalization and poor semantic understanding. LLMs, on the other hand, have shown remarkable performance in these areas due to their ability to better understand and process natural language. With well-designed prompt techniques, LLMs can effectively handle tasks such as data detection and interpolation, as demonstrated by Zhang \textit{et al.} \cite{zhang2023large}. Their research underscores LLMs' strong competency in data preprocessing through integration and semantic comprehension. Additionally, interactive systems like NL2Rigel \cite{huang2023interactive} enable users to synthesize and enhance tables from semi-structured text using natural language instructions, further illustrating LLMs' advanced data handling capabilities. Moreover, LLMs can address data scarcity by generating high-quality synthetic data. For example, a study uses an auto-regressive generative LLM to sample realistic tabular data, providing a solution where real-world data is insufficient \cite{borisov2022language}.

% Regarding information filtering and relevance determination, LLMs outperform conventional recommender systems and search engines, which typically act as passive information filters. Unlike these traditional systems, LLMs can establish the groundwork for active user engagement \cite{galitsky2024llm}, offering more dynamic and personalized filtering of information based on user inputs. Eigner \textit{et al.} \cite{eigner2024determinants} conducted a comprehensive analysis on decision-making with LLMs, demonstrating how LLMs, supported by a dependency framework, enhance the quality of decisions in human-AI collaborations. By empowering both users and organizations, LLMs contribute to more effective decision-making processes, adding value through their ability to prioritize and determine relevance in complex information streams.

% In general, LLMs show advanced competencies in information processing, particularly in integrating and synthesizing data, and in filtering and determining relevance of information. Their ability to understand and generate natural language at scale provides them with an edge over traditional models, enabling more dynamic, accurate, and effective handling of large and complex data sets.


% Contextual adaptation in LLMs, a critical aspect of executive functioning, involves the ability to adjust strategies and actions in response to evolving task demands and changing circumstances. This skill is essential for LLMs to handle real-world scenarios that require flexibility, strategic thinking, and responsive decision-making. Recent research has highlighted both the strengths and limitations of LLMs in this area, focusing on their capacity to operate in dynamic and unpredictable environments.




\subsection{Interpersonal Communications}
% Social Interaction refers to the ability of LLMs to understand, simulate, and participate in human-like social behaviors. These capabilities are essential for models to perform tasks that involve communication, collaboration, and understanding social dynamics within human interactions \cite{williams2023epidemic, mahowald2024dissociating, le2023uncovering}. Social Interaction in LLMs can be measured by evaluating their performance in tasks like role-playing, collaboration, and simulating group behaviors. These interactions are crucial for applications such as dialogue systems, virtual environments, and simulations of human societies.

% To assess Social Interaction capabilities, researchers typically measure three main dimensions:
% 1. Communication Skills: How effectively the model can exchange information in a human-like manner.
% 2. Collaborative Abilities: The model's ability to work with others, whether human or AI agents, to achieve shared goals.
% 2. Social Reasoning and Theory of Mind: The capacity to infer the thoughts, intentions, or emotions of others in social contexts.

% Several datasets and experimental setups are used to evaluate these aspects. Datasets like the Generative Agent Environment \cite{park2023generative} provide virtual environments where LLM-based agents can simulate everyday social behaviors. In these setups, agents interact, communicate, form relationships, and make collective decisions. Evaluations measure the believability of these behaviors, focusing on how well agents coordinate and respond to each other's actions. For example, in sandbox environments inspired by games like The Sims, agents simulate realistic social dynamics, such as planning a Valentine's Day party, which involves inviting others, coordinating group activities, and managing relationships.

% Zhang \textit{et al.} \cite{zhang2023exploring} explore multi-agent collaboration in their Machine Society framework, where LLM agents exhibit traits like overconfidence or easy-going personalities. These traits affect how the agents collaborate on complex tasks. Using benchmark datasets such as MMLU and Chess Move Validity, the authors found that multi-agent societies exhibit human-like behaviors, such as consensus building and conforming to group decisions, which resonate with social psychology theories. This framework also reveals that varying agent traits can affect the efficiency of collaboration, providing insights into how different social behaviors emerge in agent societies.

% Li \textit{et al.} \cite{li2023metaagents} introduced MetaAgents, a framework that situates LLM-based generative agents in task-oriented social interactions, such as a simulated job fair. In this context, agents demonstrate behaviors like interviewing, recruiting, and task coordination. Their framework combines communication, memory, reasoning, and execution modules to emulate human social dynamics. The evaluation of MetaAgents shows promising results in simulating human-like social coordination, though challenges remain when the complexity of the environment increases, especially in tasks requiring dynamic teamwork.

% Additionally, role-playing has been used as an important method for testing Social Interaction in LLMs. Shanahan \textit{et al.} \cite{shanahan2023role} examined how LLMs can be prompted to role-play different personas, allowing for the simulation of complex social interactions. For instance, by prompting LLMs to take on the roles of various characters, they can simulate deception, persuasion, and conflict resolution. This capability is essential for applications in training simulations, where realistic social interactions are necessary, such as interview preparation or negotiation training.

% Social reasoning, especially in the context of Theory of Mind(ToM), is another critical dimension for evaluating Social Interaction. Strachan \textit{et al.} \cite{strachan2024testing} tested LLMs' ability to infer others' beliefs and intentions through ToM tasks. Their findings suggest that models like GPT-4 can perform at human levels in certain ToM tasks, such as understanding indirect requests or false beliefs. However, LLMs still struggle with more nuanced social tasks like recognizing faux pas, highlighting areas where social reasoning in LLMs can be improved.

% In another study, Chuang \textit{et al.} \cite{chuang2024wisdom} evaluated the collective intelligence of LLM-based agents in political discussions. By role-playing partisans in a simulated environment, LLMs displayed human-like biases but also demonstrated the ability to converge on more accurate beliefs through deliberation, replicating the wisdom of crowds effect seen in human groups. These experiments reveal that LLMs can participate in social interactions involving group decision-making and belief updating, making them valuable tools for simulating collective behaviors in social settings.

% Overall, the Social Interaction capabilities of LLMs are advancing rapidly, with models increasingly able to simulate human-like social behaviors across various domains. Through collaborative simulations, role-playing, and theory of mind tasks, LLMs are becoming more adept at understanding and interacting with complex social dynamics, making them highly useful for a wide range of applications from virtual environments to social simulations.

emotional intelligence


% Emotional intelligence (EI) in LLMs is a crucial component of their social skills, enabling them to recognize, understand, and respond appropriately to the emotions of users. Within the emerging field of "machine psychology," which applies principles from human psychology to AI systems~\cite{hagendorff2023machine}, EI enhances human-computer interactions by facilitating empathetic communication and engaging responses that resonate with users' emotional states.

% EI can be categorized into key components relevant to social interactions: emotion perception, emotion cognition, and emotion expression. These components are essential for effective interpersonal communication, allowing LLMs to interpret emotional cues and navigate social contexts adeptly.
% To assess EI in LLMs, researchers employ psychometric tools similar to those used in human evaluations. Benchmarks like EIBENCH~\cite{zhao2024both} and EmoBench~\cite{sabour2024emobench} provide datasets specifically designed to test the EI of LLMs by focusing on these social dimensions. EIBENCH evaluates EI through tasks such as emotion recognition, cause reasoning, and empathetic response generation, which are crucial for understanding and participating in social interactions. Similarly, EmoBench assesses emotional understanding and application in complex, real-world social scenarios, testing the models' ability to engage in deep emotional reasoning within social contexts.

% Zhao \textit{et al.}~\cite{zhao2024both} introduced the Modular Emotional Intelligence enhancement method (MoEI) to improve LLMs' EI without compromising their general intelligence (GI). This approach enhances emotional perception, cognition, and expression—key for social interactions—while maintaining performance in broader reasoning tasks. Their experiments demonstrated that models like Flan-T5 and LLaMA-2-Chat could effectively balance EI and GI, showing improvements in empathy and emotional reasoning essential for social communication.

% Wang \textit{et al.}~\cite{wang2023emotional} developed the SECEU test to evaluate emotion understanding in LLMs, focusing on emotion recognition and interpretation in social contexts. This psychometric evaluation revealed that models like GPT-4 could outperform many human participants in emotional understanding, achieving accuracy scores nearing top human levels in various social scenarios.

% Elyoseph \textit{et al.}~\cite{elyoseph2023chatgpt} used the Levels of Emotional Awareness Scale (LEAS) to evaluate ChatGPT's emotional intelligence. Their findings suggest that ChatGPT outperformed the average human participant in emotional awareness and improved over time through iterative learning. This highlights LLMs' capacity for rapid improvement in EI-related tasks, enhancing their usefulness in applications requiring social sensitivity, such as mental health support and emotional diagnostics.

% At the core of emotional intelligence is the ability to apply emotional understanding in real-world social scenarios. The EmoBench framework introduced by Sabour \textit{et al.}~\cite{sabour2024emobench} evaluates not only emotion recognition but also emotional application, testing how well models facilitate decision-making and emotional regulation in socially complex and emotionally charged contexts. Despite advancements, current LLMs like GPT-4 still fall short of human-level performance in these tasks, indicating a gap in their social reasoning capabilities.

% In summary, emotional intelligence is a critical aspect of LLMs' social skills, containing emotion perception, cognition, and expression. Through comprehensive evaluations using tools like EIBENCH and EmoBench, researchers are gaining insights into how well models simulate human emotional understanding and empathy in social interactions. While LLMs show remarkable progress in emotional awareness, challenges remain in their ability to apply this emotional knowledge in complex, real-world social scenarios, which is essential for nuanced social communication.


collaboration

% LLM collaboration capabilities span two critical domains: working alongside AI agents and collaborating with human partners. These areas represent different aspects of how LLMs contribute to teamwork, strategic planning, and task execution, yet each has distinct challenges and benchmarks for evaluation.

% LLM collaboration within multi-agent systems (MAS) has shown promising advancements, particularly in optimizing task execution and strategic decision-making. In multi-agent environments, LLMs like GPT-3.5, GPT-4, and Claude-3 have demonstrated improved competencies when integrated into frameworks designed for AI-to-AI interactions. For instance, frameworks like the Dynamic LLM-Agent Network (DyLAN) enhance collaboration by allowing multiple LLM agents to share knowledge, plan strategies, and adjust to task requirements. DyLAN improves reasoning and task execution by up to 13\% through shared decision-making in reasoning and code generation tasks, as noted by Liu \textit{et al.}~\cite{liu2023dynamic}.

% Similarly, the Reinforced Advantage (ReAd) framework, introduced by Zhang \textit{et al.}~\cite{zhang2024towards}, is designed to optimize multi-agent collaboration in simulated environments. ReAd improves efficiency by implementing a closed-loop feedback mechanism that refines actions based on learned advantage functions. In this setup, LLMs are tasked with generating strategic plans and refining them through interaction, demonstrating substantial improvements in performance compared to traditional collaboration methods. However, despite these advancements, LLMs still exhibit limitations in fully matching the complex, adaptive teamwork observed in human-AI collaborations.

% The LLMARENA benchmark~\cite{chen2024llmarena} evaluates LLM collaboration capabilities in dynamic, multi-agent environments, assessing key skills such as strategic planning, communication, and opponent modeling. In tasks across seven distinct gaming environments, LLMs perform relatively well but continue to fall short of human agents in real-time adaptability and teamwork. LLMARENA uses the TrueSkill™ scoring system to gauge LLM abilities in various collaborative settings, revealing both the potential and limitations of LLMs in cooperative tasks.

% When collaborating with humans, LLMs support decision-making and task execution by providing insights, generating suggestions, and sharing knowledge. While LLMs demonstrate growing competency in assisting humans with tasks like planning and problem-solving, they still struggle with the adaptability and contextual awareness necessary to fully integrate into human teams, particularly in nuanced, culturally sensitive, or unpredictable environments.

% Human-LLM collaboration frameworks focus on improving decision-making processes and enhancing task execution by integrating LLMs into human workflows. In collaborative settings, LLMs like GPT-4 contribute to tasks like resource management, negotiation, and creative problem-solving. However, despite their capacity to generate useful insights, LLMs frequently struggle with the contextual understanding and flexibility that human partners provide. For instance, the GOVSIM platform~\cite{piatti2024cooperate} evaluates LLMs’ success in collaborative resource management tasks, where human teams often outperform LLMs in maintaining strategic adaptability.

% The RoCoBench~\cite{zhang2024towards} benchmark assesses LLM collaboration with humans in dynamic environments. It focuses on the success rate, strategic reasoning, and number of interaction steps taken by LLMs to collaborate effectively. While frameworks like the ReAd framework show some promise in improving LLM performance, RoCoBench highlights the gap between human-level strategic collaboration and the more rigid task execution of LLMs.

% Despite progress, LLMs face significant limitations in collaboration with both AI agents and humans. In AI-agent interactions, they lack the contextual understanding and flexibility needed for dynamic environments, where human reasoning excels. In human collaboration, LLMs struggle to grasp nuanced social cues essential for decision-making and teamwork.

% To address these gaps, future work should focus on enhancing LLMs' ability to incorporate real-time feedback and adapt strategies. Benchmarks like LLMARENA and RoCoBench highlight that while LLMs are improving in structured tasks, they still require better adaptability and strategic reasoning to match human-level collaboration.

% ----

% Collaboration competency in LLMs are becoming critical for multi-agent systems (MAS) and complex task optimization. Research highlights both the advancements and challenges in making LLMs work efficiently in collaborative environments, especially when compared to human performance. Studies focus on improving LLM collaboration through frameworks that facilitate agent communication, strategic decision-making, and task efficiency.

% LLMs like GPT-3.5, GPT-4, and Claude-3 have demonstrated improvements in cooperative tasks when integrated into frameworks like the Extended Coevolutionary (EC) and Dynamic LLM-Agent Network (DyLAN). These frameworks optimize multi-agent interactions by enhancing strategy formation, task management, and decision-making capabilities \cite{de2023emergent, liu2023dynamic}. DyLAN, for instance, improves performance by up to 13\% in reasoning and code generation tasks by allowing multiple LLM agents to share information and collaborate effectively \cite{liu2023dynamic}.

% Similarly, Zhang \textit{et al.} \cite{zhang2024towards} introduce the Reinforced Advantage (ReAd) framework, designed to make LLMs more efficient in multi-agent collaborations, particularly in simulated environments. ReAd improves LLMs' ability to generate strategic plans by introducing a closed-loop feedback mechanism that refines their actions based on learned advantage functions. This framework outperforms traditional methods in both efficiency and success rate, demonstrating its potential for enhancing LLM collaboration in complex, dynamic tasks.

% Multi-LLM collaboration methods, such as COOPERATE and COMPETE, improve the reliability of LLMs in handling knowledge gaps. By pooling knowledge from models like GPT-4 and Mistral-7B, these approaches increase accuracy and reduce the risk of LLMs providing incorrect information \cite{feng2024don}. This method enhances collaboration between LLMs, making them more effective in scenarios requiring diverse inputs and avoiding the issue of hallucination, which often arises in individual models.

% The LLMARENA benchmark \cite{chen2024llmarena} builds on this by evaluating LLMs in dynamic, multi-agent environments through seven distinct gaming environments, assessing crucial skills such as strategic planning, communication, opponent modeling, and team collaboration. LLMARENA uses the TrueSkill™ scoring system to provide a comprehensive evaluation of these abilities, revealing that while LLMs show potential, they continue to struggle with teamwork and opponent modeling, especially in comparison to human agents.

% Despite these advancements, LLMs continue to struggle with the adaptability and flexibility seen in human teams, particularly in unpredictable and culturally nuanced environments. LLMs, while improving in strategic planning and teamwork, lack the depth of contextual understanding that humans naturally apply in complex, real-world collaboration scenarios \cite{zhang2023exploring, piatti2024cooperate}. For example, in resource management tasks in the GOVSIM platform, LLMs like LLaMA2-70B and GPT-4 achieve limited success in maintaining sustainable outcomes, a task where human teams outperform in strategic adaptability \cite{piatti2024cooperate}.

% Several benchmarks evaluate LLM collaboration. Zhang \textit{et al.} \cite{zhang2024towards} introduce the Difficult Variants of RoCoBench (DV-RoCoBench) and Overcooked-AI to assess LLMs' ability to collaborate and plan in dynamic environments. These benchmarks test LLM agents on their success rates, number of interaction steps, and strategic reasoning. The ReAd framework, evaluated in these benchmarks, shows improved efficiency, bringing LLM performance closer to human-level strategic planning in collaborative tasks. Although LLMs are progressing in structured environments, further optimization is necessary for broader real-world applications.

% LLMs demonstrate promising advancements in collaboration and teamwork, particularly through frameworks like DyLAN and ReAd that enhance multi-agent interactions. While multi-LLM collaboration improves task performance and reliability, LLMs still lag behind human teams in flexibility and contextual understanding. Benchmarks like DV-RoCoBench, GOVSIM, and LLMARENA highlight the progress in LLM collaboration, but human reasoning and adaptability remain unmatched, especially in complex and unpredictable environments.
